MonoTAKD: Teaching Assistant Knowledge Distillation for Monocular 3D Object Detection

Monocular 3D object detection (Mono3D) holds noteworthy promise for autonomous driving applications owing to the cost-effectiveness and rich visual context of monocular camera sensors. However, depth ambiguity poses a significant challenge, as it requires extracting precise 3D scene geometry from a single image, resulting in suboptimal performance when transferring knowledge from a LiDAR-based teacher model to a camera-based student model. To facilitate effective distillation, we introduce Monocular Teaching Assistant Knowledge Distillation (MonoTAKD), which proposes a camera-based teaching assistant (TA) model to transfer robust 3D visual knowledge to the student model, leveraging the smaller feature representation gap. Additionally, we define 3D spatial cues as residual features that capture the differences between the teacher and the TA models. We then leverage these cues to improve the student model's 3D perception capabilities. Experimental results show that our MonoTAKD achieves state-of-the-art performance on the KITTI3D dataset. Furthermore, we evaluate the performance on nuScenes and KITTI raw datasets to demonstrate the generalization of our model to multi-view 3D and unsupervised data settings. Our code is available at https://github.com/hoiliu-0801/MonoTAKD.

==> custom_environment.tex <==
\def \submission {}


\usepackage{xspace}
\usepackage[dvipsnames]{xcolor}
\usepackage{comment}
\usepackage{lipsum}

\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\newcommand{\dummyfig}[1]{
  \centering
  \fbox{\centering{#1}}
}


\def\eg{\emph{e.g}\onedot} 
\def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} 
\def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot} 
\def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} 
\def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} 
\def\dof{d.o.f\onedot}
\def\iid{i.i.d\onedot} 
\def\wolog{w.l.o.g\onedot}
\def\etal{\emph{et al}\onedot}

\usepackage{listings}
\usepackage{float}

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}

\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\ttfamily\footnotesize,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2
}

\lstset{style=mystyle}

\newfloat{lstfloat}{htbp}{lop}
\floatname{lstfloat}{Algorithm}
\def\lstfloatautorefname{Algorithm}

\lstdefinestyle{myverbatim}{
    basicstyle=\ttfamily\footnotesize,
    backgroundcolor=\color{white},
    breaklines=true,
    breakatwhitespace=true
}

\definecolor{Crimson}{rgb}{0.86, 0.08, 0.24}
\definecolor{DarkGreen}{rgb}{0.00, 0.40, 0.00}
\definecolor{RoyalBlue}{rgb}{0.25, 0.35, 0.74}
\definecolor{DarkCyan}{rgb}{0.0, 0.54, 0.54}
\definecolor{Gray}{gray}{0.95}
\definecolor{ChromeYellow}{rgb}{1.0, 0.65, 0.0}
\definecolor{Red}{rgb}{1.0, 0.0, 0.0}

\ifx \submission \undefined
\newcommand{\wu}[1]{\textcolor{DarkGreen}{#1}}
\newcommand{\yyy}[1]{\textcolor{RoyalBlue}{#1}}
\newcommand{\xxx}[1]{\textcolor{DarkCyan}{#1}}
%\newcommand{\todo}[1]{\textcolor{Red}{#1}}
\else
% do NOT display comments
\newcommand{\wu}[1]{{#1}}
\newcommand{\yyy}[1]{{#1}}
\newcommand{\xxx}[1]{{#1}}
%\newcommand{\todo}[1]{{#1}}
\fi

==> sec/Checklist.tex <==
\section{Reproducibility Checklist}

% Checklist macros
\newcommand{\answerYes}[1]{\textcolor{blue}{#1}} 
\newcommand{\answerNo}[1]{\textcolor{teal}{#1}} 
\newcommand{\answerNA}[1]{\textcolor{gray}{#1}} 
\newcommand{\answerTODO}[1]{\textcolor{red}{#1}} 

\begin{enumerate}

\item This paper
\begin{enumerate}
%  (yes/partial/no/NA)
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced? \answerYes{Yes.}
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results? \answerYes{Yes.}
    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper? \answerYes{Yes.}
\end{enumerate}

\item Does this paper make theoretical contributions? \answerYes{No.} If yes, please complete the list below.
\begin{enumerate}
    \item All assumptions and restrictions are stated clearly and formally. \answerYes{Yes.}
    \item All novel claims are stated formally (e.g., in theorem statements). \answerYes{Yes.}
    \item Proofs of all novel claims are included. \answerYes{Yes.}
    \item Proof sketches or intuitions are given for complex and/or novel results. \answerYes{Yes.}
    \item Appropriate citations to theoretical tools used are given. \answerYes{Yes.}
    \item All theoretical claims are demonstrated empirically to hold. \answerYes{Yes.}
    \item All experimental code used to eliminate or disprove claims is included. \answerYes{Yes.}
\end{enumerate}

\item Does this paper rely on one or more datasets? \answerYes{Yes.} If yes, please complete the list below.
\begin{enumerate}
    \item A motivation is given for why the experiments are conducted on the selected datasets \answerYes{Yes.}
    \item All novel datasets introduced in this paper are included in a data appendix. \answerYes{NA.}
    \item  All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \answerYes{NA.}
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. \answerYes{Yes.}
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. \answerYes{Yes.}
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. \answerYes{NA.}
\end{enumerate}

\item Does this paper include computational experiments? \answerYes{Yes.} If yes, please complete the list below.
\begin{enumerate}
    \item Any code required for pre-processing data is included in the appendix. \answerYes{Yes.}
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. \answerYes{Yes.}
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \answerYes{Yes.}
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from \answerYes{Yes.}
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. \answerYes{NA.}
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. \answerYes{Yes.}
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. \answerYes{Yes.}
    \item This paper states the number of algorithm runs used to compute each reported result. \answerYes{Yes.}
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. \answerYes{Yes.}
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank).  \answerYes{Yes.}
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. \answerYes{Yes.}
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. \answerYes{Yes.}
\end{enumerate}

\end{enumerate}

==> tab/tab_diff_teacher.tex <==
\begin{table}[t]
\centering
\caption{Compares the performance boost using different teacher models on the KITTI \textit{val} set. Impro. indicates the $AP_{3D}$ and $AP_{BEV}$ improvements.}
% \resizebox{0.8\linewidth}{!}{
\begin{tabular}{l|ccc|ccc}
\hline
\multirow{2}{*}{Settings} &  \multicolumn{3}{c|}{$AP_{3D}$}    & \multicolumn{3}{c}{$AP_{BEV}$} \\              
% \cline{2-7}
                          & Easy & Mod. & Hard    & Easy & Mod. & Hard    \\ \hline
Baseline      & 24.35 & 16.16 & 13.44 & 31.78 & 21.61 & 18.80 \\ \hline
w/ Centerpoint~\cite{centerpoint}   & 27.06 & 19.38 & 17.50 & 35.66 & 26.03 & 23.09 \\ 
Impro.               & 2.71 & 3.22 & 4.06 & 3.88 & 4.42 & 4.29  \\ \hline
w/ Pointpillar~\cite{pointpillar}   & 31.28 & 20.80 & 17.58 & 42.21 & 28.48 & 24.73 \\ 
Impro.                    & 6.93 & 4.64 & 4.14 & 10.43 & 6.87 & 5.93 \\ \hline
w/ Second (Ours) & \textbf{34.36} & \textbf{22.61} & \textbf{19.88} & \textbf{42.86} & \textbf{29.41} & \textbf{26.47} \\ 
Impro.                    & ~\textbf{10.01} & \textbf{6.45} & \textbf{6.44}~ & ~\textbf{11.08} & \textbf{7.80} & \textbf{7.67}~ \\ \hline
\end{tabular}
% }
\label{tab:difftea}
% \vspace{-12pt}
\end{table}

==> tab/visualization.tex <==
\begin{figure}[t]
\centering
    % Second row with three subfigures
    \begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\textwidth]{compare/cmkd_3D.png}
    \label{fig:sub4}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\textwidth]{compare/monodetr_3D.png}
    \label{fig:sub5}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\textwidth]{compare/monnotrkd_3D.png}
    \label{fig:sub6}
    \end{subfigure}
    % First row with three subfigures
    \begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\textwidth]{compare/cmkd_BEV.png}
    \label{fig:sub1}
    \caption{CMKD}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\textwidth]{compare/monodetr_BEV.png}
    \label{fig:sub2}
    \caption{MonoDETR}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\textwidth]{compare/monotrkd_BEV.png}
    \label{fig:sub3}
    \caption{\model (Ours)}
    \end{subfigure}

    \caption{Qualitative results on KITTI \textit{val} set for the Car category. We compare the qualitative results among CMKD~\cite{cmkd}, MonoDETR~\cite{monodetr}, and our proposed~\model. The first and second rows represent detection results from a frontal view camera and a bird's eye view, respectively. We use green and red boxes to indicate the ground truth and prediction bounding boxes.}
    % Note that, in the first row, 3D bounding box predictions of our~\model are shown in the perspective view. The blue circles highlight the most notable improvements compared to the other two methods
    \label{fig:3d_bev}  
\end{figure}
